Measuring Psychological Depth in Language Models

Evaluations of creative stories generated by large language models (LLMs) often focus on objective properties of the text, such as its style, coherence, and diversity. While these metrics are indispensable, they do not speak to a story's subjective, psychological impact from a reader's perspective. We introduce the Psychological Depth Scale (PDS), a novel framework rooted in literary theory that measures an LLM's ability to produce authentic and narratively complex stories that provoke emotion, empathy, and engagement. We empirically validate our framework by showing that humans can consistently evaluate stories based on PDS (0.72 Krippendorff's alpha). We also explore techniques for automating the PDS to easily scale future analyses. GPT-4o, combined with a novel Mixture-of-Personas (MoP) prompting strategy, achieves an average Spearman correlation of 0.51 with human judgment while Llama-3-70B with constrained decoding scores as high as 0.68 for empathy. Finally, we compared the depth of stories authored by both humans and LLMs. Surprisingly, GPT-4 stories either surpassed or were statistically indistinguishable from highly-rated human-written stories sourced from Reddit. By shifting the focus from text to reader, the Psychological Depth Scale is a validated, automated, and systematic means of measuring the capacity of LLMs to connect with humans through the stories they tell.

==> sections/framework_v1_sm.tex <==
% sreya's version
\section{Related Work}

Rubrics serve as a key instrument for evaluating writing, so we chose to create a set of metrics that encompass notable attributes pertinent to our study of evaluating LLMs at a psychological depth level. To come up with a list of metrics we consulted several psychology papers to get attributes that have an impact on defining what the term ‘psychological depth’ meant. After filtering and consolidating, we finalized 5 different metrics to use in our study: authenticity, empathy, engagement, emotion provoking, and narrative complexity. 

\textbf{Authenticity:} This metric focuses on asking if the writing felt true to real human experiences, regardless of whether the reader personally experienced the situation. To be authentic also targets the idea of representing a psychological process that’s believable. A study reported that narratives written authentically and inauthentically coincided with their reported self-scores\cite{Wilt2019}. This suggests that humans can clearly distinguish between authentic and inauthentic writing, which shows how important authenticity can be to an audience. 

\textbf{Empathy:} It measures how well the audience was able to empathize with the characters and their situations in the text. This also tests the possibility of the reader being able to lead to new introspection or new insights about the world. A study states how empathetic people mention a lot of negative feelings, such as feeling overwhelmed or isolation \cite{Yaden2023}. This proves that writing infused with empathy can help bond readers and writers over painful experiences which unlocks the writing piece’s ability to get readers to understand their point of view. 

\textbf{Engagement:} Choosing this measurement was important to see how well the writing piece was able to keep the reader’s focus at an emotional and psychological level. In a study, researchers were able to find a positive correlation between engaging stories and higher engagement scores, which also confirms engagement as a significant factor to use.\cite{Sukalla2015}.  

\textbf{Emotion provoking:} This measurement forces the readers in the study to distinguish between describing the nuances of a character’s state rather than using simple terms that give surface-level writing. The significance of the metric on one’s psychological state can be seen in a study such that shows that writing about emotional experiences show significant improvement on mental and physical health\cite{Pennebaker1997}. This proves that using emotion-provoking is a key component in evaluating psychological depth as it directly correlates to mental health. 

\textbf{Narrative complexity:} Using narrative complexity as a metric in this study puts a lens on characters having multifaceted personalities and exhibiting internal conflicts. Stories should also aim to explore more complicated relationships between characters rather than stereotypical ones. A study points out how films evoke dissonant cognitions in their audience\cite{Kiss2017}. This is a clear indicator of the possible mental effects the style of a narrative can have. 

==> sections/framework_v2_fhc.tex <==
\section{The Psychological Depth Scale}

To comprehensively assess the psychological depth of LLMs through their narrative generations, we established a Psychological Depth Scale (PDS) predicated on key metrics derived from an extensive literature review within cognitive science, psychology, film studies, and narrative analysis. These metrics are designed to measure five related but separable aspects of psychological depth in stories: authenticity, emotion provocation, empathy, engagement, and narrative complexity. 

\textbf{Authenticity (AUTH)} describes whether narratives convey events and thought processes that resonate as true to human experiences, even if they are not universally shared. Its significance is well documented in philosophy and psychological research connecting authenticity to personal well-being \cite{multicomponent_authenticity, robinson2013authenticity}. Research in public communication has also demonstrated that narratives enriched with realistic contexts help establish credibility and enhance persuasive impact \cite{petraglia2009importance}. It is therefore pivotal to ensure stories feel personal and reflective of real-life complexities.

\textbf{Emotion Provocation (PROV)} measures the narrative's ability to elicit strong emotional responses, whether positive or negative. The relevance of this component to psychological depth is evidenced by studies demonstrating that text with high \emph{valence} (the pleasantness of a stimulus) and \emph{arousal} (the intensity of emotion provoked) directly influence memorability \cite{memorability1999}, reading efficiency and comprehension \cite{comprehension2015, comprehension2019}. 

\textbf{Empathy (EMP)} refers to the ability to effectively recognize and respond to the emotions of other persons \cite{empathy_vs_transport2013}. Empathetic narratives instill concern for unfortunate others and catalyze personal introspection that can lead to more prosocial behavior \cite{empathy_prosocial2008}, emotional intelligence \cite{emotional_intel_empathy}, and broader insights into the human experience \cite{empathy1980, empathy2010}. Thus, the moral benefits of a story's ability to arouse empathy make it an important dimension to consider in our framework for evaluating creative generation. 

\textbf{Engagement (ENG)} assesses the ability of a story to captivate and maintain a reader's attentional focus \cite{measuring_engagement2009}. Roughly analogous to the psychological concept of \emph{transportation} \cite{transportation1993}, an engaged reader is more likely to lose track of time and fail to observe events going on around them \cite{engagement2008}. If a story's world is distant from the one in which the reader lives, engagement can reinforce an integrated perception of that world within the story context, even when events would not otherwise be possible in reality. When a reader is not able to identify with a fictional narrative or its characters and does not become transported or engaged, this can lead the reader to become distracted or frustrated \cite{empathy_vs_transport2013}. 

\textbf{Narrative Complexity (NCOM)} examines the intricacy of character and plot developments beyond common stereotypes and tropes as well as the vividness of narrative descriptions \cite{development2018}. \citet{Kiss2017} show that writers can also create more immersive experiences by strategically deploying complexity via deliberate confusion, paradoxes, and unresolved ambiguities. Prior work exploring the psychological structure of creative writing also highlights that non-linear and metaphorical elements strongly contribute to perceptions of narrative quality \cite{psychological_structure}.

==> sections/framework_v3_zy.tex <==
\section{The Psychological Depth Scale}

% this is where the lengthy version of the section will live!
% last removals from the final version are added in the following few lines:
%  removed from the first par:
% FHC: reducing some of the citations to save space. 
% The practical advantages of both frameworks are observed across education and literary training \cite{woodruff_etal_2017,kunjanman2021,bouguelmouna_benzoukh2022,iskhak_etal_2017}, translation studies \cite{tian_wang2019,chan2016,maatoq_kadhim2019}, and consumer research \cite{scott1994,kushneruk2017}. 
%ZY: given the new simplifications the flow is better when the following is removed per pengnanyun's suggestion: "By eliminating “the subject-object dichotomy”, reader-response approaches validate subjective reader experiences as part of a larger, intersubjective framework of narrative analysis \cite{fish1980}." 
%  removed from emotion prov:
%FHC: Removing this because it doesn't add too much and it interrupts  the continuity about valence going into the next paragraph
% The cognitive impact of emotional provocation has largely been established in concept formation, information processing, and memorization \cite{wilsonmendenhall_barsalou2016, knickerbockeretal2015, Knickerbocker_etal2014}. 
%  prev. empathy:
% FHC: preserving original citations, but cutting some out for length
% \textbf{Empathy (EMP)} captures narrative evocation of empathetic responses in readers, such as immersive identification with characters and cognitively partaking in narrated experiences \cite{miall_kuiken2001} \cite{oatley2002} \cite{escalas_stern2003} \cite{zaki_ochsner2012}. The neural and cognitive structure of empathy and its social and psychological impact is well-documented in the literature \cite{davis1994} \cite{decety_jackson2004} \cite{Hoffman1991} \cite{uddin_etal2007} \cite{ShamayTsoory_etal2008}. Both behavioral studies and fMRI research demonstrate that empathetic identification facilitates a cognitive deployment shift in readers, privileging fictional perspective over one's own perspective \cite{kaufman_libby2012} \cite{bower_morrow1990} \cite{speer_etal2009} \cite{trabasso_chung2004}. Narratively evoked empathetic responses catalyze introspection and perspective-taking, facilitating prosocial behavior \cite{empathy_prosocial2008}, emotional intelligence \cite{emotional_intel_empathy}, and insight into the human experience \cite{empathy1980, empathy2010} \cite{singer_etal2006}. Emphathetic narratives embody “suggestion structure[s]” that conjure up themes of shared human experiences through the use of tropes such as metaphor and metonymy \cite{oatley2002} \cite{JohnsonLaird_oatley2016}. Narrative evocation of empathy is therefore a plausible indicator of psychological depth of stories. 
%  removed from authenticity:
% FHC: Removing this for now, I think it's too much for NLP people
% A cognitive-philosophical meta-analysis describes authenticity as involving self-awareness and “unbiased processing of self‐relevant information”, as well as exhibiting the behavioral and social-relational outputs of these aspects \cite{kernis_goldman2006}.

We established a Psychological Depth Scale (PDS) to comprehensively assess the psychological depth of LLMs through their narrative generations. PDS is predicated on key metrics that are derived from an extensive literature review within cognitive science, psychology, film studies, and narrative analysis. The choice of metrics is underpinned by two reader-centered theoretical frameworks: reader-response criticism and text world theory (Fish 1938, 1970; Canning 2017; Babaee and Montashery 2012;  Bell et al. 2019; Cushing 2017; Gavins 2007; Mailloux 1976).

Reader-response theory is a school of literary criticism that centers the role and experience of the reader in narrative analysis. Stanley Fish, a forerunner of the tradition in the direction of affective stylistics, summarizes the methodology as replacing the question “what does this sentence mean?” by “what does this sentence do?” (Fish, 1970, p. 125). Fish suggests that “interpretive communities” marked by shared interpretive strategies are solely responsible for meaning production (Fish, 1980, p. 14). Consequently, they are the source of formal textual patterns and even the limits of mental operations individuals can perform (Fish, 1980, p. 14). By eliminating “the subject-object dichotomy”, subjective reader experiences are validated as part of a larger intersubjective framework of narrative analysis. 

Text world theory has roots in the late 20th-century developments in AI, cognitive psychology, and philosophy of mind (Gavins 2007). The text-world framework goes beyond textual construction and focuses on the influence of the “discourse-world” (contextual and situational elements) on how the language is produced and received (ibid., pp. 8-9). Humans communicating within the discourse-world simultaneously construct “text-worlds”, which are “mental representations of the discourse” facilitating language comprehension (ibid., p. 10). Text-worlds result from rule-governed world-building: possible models of reality are dynamically constructed and evaluated as new information is presented (ibid., p. 36). 

We conducted a comprehensive search on several databases, including Google Scholar, PubMed, and JSTOR. Our search terms included “psychological depth in literary texts”, “cognitive narrative analysis”, and “reader-response theory”. The results of the initial search were screened for discussion and application of text-oriented evaluative criteria for narrative quality and facilitation of reader-response. 95 peer-reviewed articles and books were included in the final review. 143 evaluative components were extracted from the included works. We employed thematic analysis to group these candidates under five metacomponents: emotion provocation, empathy, engagement, authenticity, and narrative complexity. The metrics of PDS are designed to measure these five related but distinct components of psychological depth in stories. 

Below we review the significance of each chosen metric for PDS, and discuss how each may be achieved in a story. It is worth noting that while factors contributing to each metric may be complex, measuring the extent of their narrative achievement is relatively simpler.  As PDS is a reader-centered assessment tool, each metric is such that readers will know when a story achieves it.  Our surveys reflect this fact.

\textbf{Emotion Provocation (PROV)} measures the narrative’s ability to elicit strong emotional responses, positive or negative.   
Theories of emotions range across neuroscience %(Neural Fingerprinting: Meta-Analysis, Variation, and the Search for Brain-Based Essences in the Science of Emotion -- Clark‑Polner, Wager, Satpute, and Barrett; Emotion and the Autonomic Nervous System -- Mendes; Anderson and Adolphs 2018, Dalgleish 2004)
, cognitive psychology %(Ortony, Clore, and Collins 1988), (Lazarus 1991), (Oatley and Johnson-Laird 2014)
, and philosophy (Sartre 1939; Nussbaum 2004). Contemporary approaches generally describe emotions as intentional (object-directed) evaluative mental states marked by valence (degree of salient positivity or negativity) and arousal (level of intensity) (Barrett, Lewis, and Jones 2016). 

Emotional states influence the experience of reading stories before (choice of book), during (narrative evocation of emotions and memories, impacting attention and engagement), and after (persistence and/or recurrence of evoked emotions) the experience 
%(Mar , Oatley , Djikic, Mullin 2011 Emotion and narrative fiction: Interactive influences before, during, and after reading, Cognition & Emotion, 25:5, 818-833, DOI: 10.1080/02699931.2010.515151)
The impact of emotion provocation on reader cognition has largely been established in areas of concept formation, reading comprehension, information processing, and memorization 
%A Fundamental Role for Conceptual Processing in Emotion -- Christine D. Wilson‑Mendenhall and Lawrence W. Barsalou
%Emotion effects during reading: Influence of an emotion target word on eye movements and processing. Cognition and Emotion, 29(5), 784–806. https://doi.org/10.1080/02699931.2014.938023 
%Reader reaction to news of mass suffering: Assessing the influence of story form and emotional response. Journalism, 18(8), 1011-1029. https://doi.org/10.1177/1464884916663597
%Knickerbocker, H., Johnson, R. L., & Altarriba, J. (2014). ; Maier, S. R., Slovic, P., & Mayorga, M. (2017). 

Recent fMRI research shows that emotive expressions in text are more cognitively effective for the reader when valence and arousal are \textit{congruent} (positive valence - high intensity, negative valence - low intensity) as opposed to \textit{conflicting} (positive valence - low intensity, negative valence - high intensity). %[Emotional valence and arousal affect reading in an interactive way: neuroimaging evidence for an approach-withdrawal framework. (Citron, F. M., Gray, M. A., Critchley, H. D., Weekes, B. S., & Ferstl, E. C. (2014).] ;  [Megalakaki, Olga  and Ballenghein, Ugo  and Baccino, Thierry 2019] ; 
Such cognitive impact disparity between congruent and conflicting narrative emotions may be a factor in "compassion fatigue" (Maier 2015; 2016; Kinnick et al. 1996) and "psychic numbing" (Maier et al. 2016; Barnes et al. 1999; Slovic et al. 2013) exhibited by news readers in the face of mass tragedies. 
%Kinnick KN, Krugman DM and Cameron GT (1996) Compassion fatigue: Communication and burnout toward social problems. Journalism & Mass Communication Quarterly 73: 687–706. 
%Friedrich J, Barnes P, Chapin K, et al. (1999) Psychophysical numbing: When lives are valued less as the lives at risk increase. Journal of Consumer Psychology 8(3): 277–299.
%Slovic P, Zionts D, Woods AK, et al. (2013) Psychic numbing and mass atrocity. In: Shafir E (ed.) The Behavioral Foundations of Policy. Princeton, NJ: Princeton University Press,pp. 126–144.
Enhancing a story's emotional impact is therefore a task more complex than simply increasing the amount and intensity of emotion-laden content as this may elicit weaker emotional responses from readers. Given the impact and complexity of emotion provocation, we contend that emotional provocation is an achievement of psychologically deep stories and thereby a crucial metric in narrative quality assessment of stories. 

\textbf{Empathy (EMP)} broadly captures narrative evocation of empathetic responses consisting of complex emotional and cognitive states %(Miall & Kuiken, 2002; Oatley, 2002; Escalas & Stern 2003). 
Empathy is the ability and tendency to cognitively partake in emotions and thought-processes of others (Zaki & Ochsner, 2012). Empathy as a distinctive cognitive category is well-documented in the literature %(Davis, 1994; Decety & Jackson, 2004; Hoffman 1984; Singer, 2006; Uddin, Iacoboni, Lange, &Keenan, 2007), (Shamay-Tsoory, Aharon-Peretz, & Perry,2009) (Davis, 1983). 
Empathetic responses consist in feeling \emph{as} another, whereas sympathy is feeling \emph{for} another through remembered emotions %(JohnsonLaird & Oatley, 2008; Escalas & Stern 2003; Maier, Slovic, & Mayorga 2017).

Empathetic narratives facilitate reader identification with narrated characters and/or the narrator (Johnson Laird and Oatley 2016, ). Both behavioral studies and fMRI research demonstrate that empathetic identification facilitates a cognitive deployment shift in readers, privileging fictional perspective over one's own perspective %(Kaufman and Libby 2012; Bower & Morrow, 1990; Speer, Reynolds, Swallow, & Zacks, 2009; Trabasso and Chung 2004). 
Narratives evoking empathetic responses catalyze introspection and perspective-taking that can lead to more prosocial behavior \cite{empathy_prosocial2008}, emotional intelligence \cite{emotional_intel_empathy}, and broader insights into the human experience \cite{empathy1980, empathy2010}. 

Psychologically deep narratives possess “suggestion structure[s]” that drive empathetic responses in the reader (Oatley 2002). Such structures involve tropes such as metaphor and metonymy, psychologically suggestive of intended themes and shared human experiences (Johnson Laird and Oatley 2016). Evocation of empathy is therefore an integral component of psychological depth in narrative stories. 

\textbf{Engagement (ENG)} assesses the ability of a story to captivate and maintain a reader's attentional focus \cite{measuring_engagement2009}. Narrative engagement is a major component of \emph{transportation} \cite{transportation1993}, whose positive social and cognitive effects have been established (Johnson 2012, Green et al. 2008). As transportation consists of engagement and emotional response (Green et al. 2008), we have chosen to treat each component separately. 

Engagement in a narrative can facilitate “enduring persuasion and strong attitudes” in readers (Green 2008, p. 530). Relatedly, how much fun is experienced in a fictional setting is a matter of how engaged the participant is (Goffman p. 161). More engaged readers are more likely to lose track of time and fail to notice changes in their surroundings \cite{engagement2008}. In contrast, fictional narratives unable to draw engagement may distract or frustrate the reader \cite{empathy_vs_transport2013}. These results reveal the reciprocal role of engagement in stories both as a precursor for other narrative achievements and as a measure of them. 

\textbf{Authenticity (AUTH)} describes the extent to which a narrative text reflects expressions of genuine human experiences and emotions, albeit not universally shared. In philosophy, authentic expressions are claimed to manifest one’s natural self (Rousseau 1754, 1761, 1770), construct one’s identity over time (Kierkegaard 1849), and capture what it means to exist in the world as a human being in relation to oneself and others (Heidegger 1927; Berlin 2000; Taylor 2003; Gerrig 1993). Kernis and Goldman adopt a combined philosophical and psychological approach, defining authenticity as “the unobstructed operation of one’s true‐ or core‐self in one’s daily enterprise” (2016, p. 294). In their analysis, authenticity involves cognitive self-awareness and “unbiased processing of self‐relevant information”, as well as exhibiting the behavioral and social-relational outputs of these aspects (p. 294; p. 296; p. 298; p. 300). 

Studies in psychology, media studies, and communication theory suggest that positive authenticity judgments help fulfill a social “need to belong” (Newman and Smith 2011; 2016), that narratives enriched with realistic contexts help establish credibility and enhance persuasive impact \cite{petraglia2009importance}, and that higher levels of perceived realism reflected in stories contribute to higher levels of reader and viewer engagement (Busselle & Bilandzic, 2007; Green, 2004; Hall, 2003; Zhang, Hmielowski, & Busselle, 2007). Authenticity is therefore a major component in narrative quality. 

Psychologically deep stories convey authentic aspects of human existence the reader could resonate with, and even “feel one’s way in” (Einfühlung) when depictions involve “radical mental difference” (Forster 2022 -- Stanford encyc. of phil. entry on Herder https://plato.stanford.edu/entries/herder/ ). Thus, authenticity as a measure of psychological depth in stories underscores the importance of ensuring that stories feel personal and reflective of real-life complexities.


\textbf{Narrative Complexity (NCOM)} refers to the presence of a rich and intricate web of storylines and character development that derives puzzled interest and cognitive commitment from the reader \cite{development2018}. Writers achieve narrative complexity by deploying innovative and creative storytelling techniques such as nonlinear or multilinear narration, plot twists, and double perspectivation \citet{Kiss2017}. 

Complex narratives present immersive puzzles that require readers to undertake mental restructuring, retroactive revision, and developing alternative interpretations \citet{Kiss2017} “Simplicity, Complexity, and Narration in Popular Movies” James E. Cutting; Zunshine 2006). Exerting cognitive effort to unravel narrative complexities facilitates reader attention and interest (“Simplicity, Complexity, and Narration in Popular Movies” James E. Cutting; Empson 1947; Steiner 1978), and renders a more enjoyable reading experience (Zunshine 2006).

Narrative complexity is distinct from narrational complexity: a simple story can be made impenetrable through an obscure narration and a complex story can be created without any complex language use (“Simplicity, Complexity, and Narration in Popular Movies” James E. Cutting). Furthermore, narrative complexity is experienced both on subjective and intersubjective levels, where intersubjectivity depends on situational and cognitive similarities of subjects (Tikka and Kaipainen 2017). Thus, narrative complexity is a dynamic and reciprocal measure that goes beyond stylistic and structural choices. 





==> tables/iaa_corrs.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccc|llll}
\toprule
   & \multicolumn{3}{c|}{\textbf{K-$\alpha$}}  & \multicolumn{4}{c}{\textbf{Correlations}} \\
\midrule
\textbf{Component}   & Human & \multicolumn{1}{l}{GPT-3.5$_{MoP}$} & \multicolumn{1}{l|}{GPT-4$_{MoP}$} & 
                               \multicolumn{1}{l}{GPT-3.5} & \multicolumn{1}{l}{GPT-3.5$_{MoP}$} & \multicolumn{1}{l}{GPT-4} & \multicolumn{1}{l}{GPT-4$_{MoP}$}\\
\midrule
AUTH       & 0.7110 & 0.9028 & 0.9206 & 0.1611  & 0.2672* & 0.3210* & 0.3796*  \\
EMP        & 0.7462 & 0.8953 & 0.9314 & 0.4809* & 0.5272* & 0.4913* & 0.5352*  \\
ENG        & 0.7065 & 0.8987 & 0.8686 & 0.0527  & 0.0976  & 0.2389* & 0.3572*  \\
PROV       & 0.7127 & 0.8970 & 0.9347 & 0.3568* & 0.4697* & 0.4171* & 0.4458*  \\
NCOM       & 0.7360 & 0.8984 & 0.8650 & 0.1266  & 0.2143* & 0.4217* & 0.4901*  \\
\midrule
\textbf{Average} & 0.7225 & 0.9041 & 0.8984 & 0.2356 & 0.3152 & 0.3780 & \textbf{0.4416} \\
\bottomrule
\end{tabular}%
}
\vspace{-1mm}
\caption{Rater agreement as measured by Krippendorff's alpha (K-$\alpha$) and Spearman Rank Correlations between human and LLMs judgments of depth. Asterisks (*) indicate significant correlations with p-values $< 0.05$.}
\vspace{-2mm}
\label{tab:iaa_corrs}
\end{table*}

==> tables/p+w_characters_output.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{\textsc{Plan+Write}'s Character Portraits Output, Premise 2}\\
\midrule
{\fontfamily{cmss}\selectfont
1. Samuel Price: Samuel, mid-thirties with disheveled brown hair and tortured blue eyes, is the primary character who is dealing with severe depression. Once a lively and creative soul, his world is now tinged with unending shades of grey. Every morning, he wakes up to the same feeling of emptiness and despair that often overpowers him into a motionless state. Thoughts of unworthiness and self-loathing are constant companions that he fails to ward off. His world has fallen silent, even amidst the chaos. However, the unexpected arrival of a creature that reflects his internal struggles so perfectly lights a flickering flame of purpose in his heart.\newline

2. Charlie: Charlie is a coal-black Labrador Retriever with soulful eyes that seem to mirror much more profound grief than any canine could be expected to bear. The furrow of his brows and his constant whimper tells a story of incessant inner turmoil that somehow seems to overshadow that of Samuel's. He barely eats, barely plays - his spirit is shattered, his life force dimmed. His existence represents an amplification of Samuel's struggles, magnifying them into something entirely unbearable, yet strangely relatable. But beneath the apparent desolation, Charlie's thoughts, even in their depressing state, are loyal towards Samuel, ensuring him that he is not alone in his battle.\newline

3. Dr. Lorraine Fisher: Dr. Fisher is the psychiatrist who ends up mixing up the paperwork, leading to Charlie's arrival into Samuel's life. Being middle-aged, she is a seasoned professional with honey blonde hair that radiates a warmth contradicting her often cold and methodical approach to her practice. She is smart, undeniably good at her job, but she hides behind an aloof persona to separate her personal emotions from her profession. Her primary struggle is dealing with the guilt of the mix-up while observing the peculiar bond growing between Samuel and Charlie. Her thoughts grapple with the ethical implications of her mistake and the unexpected positive outcome it has had on Samuel's otherwise stagnant therapy.
}\\
\bottomrule
\end{tabular}
}
\caption{\textsc{Plan+Write}'s Character Portraits Output for Premise 2.}
\label{tab:p+w_characters_output}
\end{table*}

==> tables/p+w_characters_prompt.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{\textsc{Plan+Write}'s Character Portraits Prompt}\\
\midrule
{\fontfamily{cmss}\selectfont
Premise: You are severely depressed and are given a service dog to help you through it. However, due to a mixup, you are given a dog that is actually much more depressed than you. The main thing that gets you up in the morning is knowing that you need to be the service human for your dog.\newline

Task: Based on the premise, describe the names and details of 2-3 major characters. Focus on each character's emotional states and inner thoughts.\newline

Only respond with the characters' names and descriptions.
}\\
\bottomrule
\end{tabular}
}
\caption{\textsc{Plan+Write}'s Character Portraits Prompt with an example premise.}
\label{tab:p+w_characters_prompt}
\end{table*}

==> tables/p+w_story_output.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{\textsc{Plan+Write}'s Story Composition Output, Premise 2}\\
\midrule
{\fontfamily{cmss}\selectfont
In the frosty prison of his depression, Samuel Price found himself waking every morning to the same haunting emptiness. His world, once filled with color, was now a relentless parade of greys. His life had become a hushed echo, the silence broken only by the relentless whispers of unworthiness that shrieked in his ears. \newline

Samuel's doctor, \colorbox{yellow}{Dr. Lorraine Fisher}, proposed a solution to this monotony - a service dog, a beacon of unwavering loyalty and love. Her efficient hands made a mistake, however, sending not a helper but an echo, a manifestation of Samuel's own depressions in the form of a melancholy Labrador named Charlie. Charlie wandered into Samuel's colorless world, carrying shadows deeper than his coal-black fur. \newline

For the first time in years, a jolt of feeling swept through Samuel. His heart wept at the sight of Charlie, his quiet whines and downcast gaze reflecting his own despair. Charlie was Samuel in dog form, only his depression was magnified, laid bare for the world to see. \newline

The first mornings were unsettling, the despair now tangible in the home. Samuel sat with Charlie, their mutual misery fusing into a gloomy camaraderie. But then came a slow and unexpected shift. Despite his depression mirroring Samuel's, Charlie still managed to wag his tail when Samuel came around. A spark of something, perhaps recognition, perhaps solidarity, perhaps care, stirred within Samuel's icy heart. His morning ritual shifted from waking up to the complex hell of his thoughts to getting up because he knew Charlie needed him. He was not curing Charlie's pain; he was mere company to it, like Charlie was to his.\newline

A mix-up, thought Dr. Fisher, ironing the wrinkle from her pristine form. The clinical brilliance that often sparkled in her eyes was dulled by guilt. She'd promised help, not a measly reflection of his agony. But when she saw them together, their empathetic companionship and understanding, she was taken aback. The mix-up had resulted in an accidental therapy, a living breathing support system for each other. Ethical implications marred her relief, but Samuel's progress was undeniable. \newline

Burdened yet elated by Charlie's presence, Samuel started taking small steps towards overcoming his depression. Countless days faded into each other as he made breakfast for Charlie, played fetch on his good days, and just sat by his side on bad ones. Charlie, in return, was there, silent but supportive, sharing his misery with faithful companionship. Each day was a mirror to the next, but in the shared melancholy, they found comfort, companionship, and a reason to wake up each morning.\newline

The afflicted Labrador was no cure, but his mutual agony somehow validated Samuel's despair. A sense of purpose grew from this shared pain, making each moment bearable. Samuel and Charlie became a beacon of hurt but also healing, a reflection of human-dog companionship's deeply emotional potential, and a testament to the shared strength beneath depression's cold, grey waves.\newline

One morning, Samuel smiled at Charlie, love whirling within the hollows of his exhausted heart. \"We are mirrors, buddy,\" he said, \"Reflecting each other's darkest parts and, somehow, making them a little brighter.\" In response, Charlie looked up, his mournful eyes holding a trace of warmth. His tail wagged, slow but sure - a kiss of hope in their shared gloom.\newline

Their tale was an unconventional therapy, draped in the dark cloak of depression. Yet, in the end, it was the darkness that guided them towards the light.
}\\
\bottomrule
\end{tabular}
}
\caption{ GPT-4 generated story of \textsc{Plan+Write} for Premise 2. The story follows the given promise and character portraits and is overall coherent.}
\label{tab:p+w_story_output}
\end{table*}

==> tables/premise_1.tex <==
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{Premise 1}\\
\midrule
{\fontfamily{cmss}\selectfont
You died and awoke in the afterlife. It's quite nice actually. The people and atmosphere are a lot nicer than you are used to and there is no stress or pressure. When you ask what good deed got you into heaven you are informed that this is hell, followed by a visit from a very concerned demon.}\\
\bottomrule
\end{tabular}
}
\caption{Premise 1 from Reddit’s \texttt{r\textbackslash WritingPrompts}. The premise provides basic background information for the characters and setting of a story. Details of the characters, including their inner states, are not mentioned.}
\label{tab:premise_1}
\end{table*}

==> tables/premise_2.tex <==
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{Premise 2}\\
\midrule
{\fontfamily{cmss}\selectfont
You are severely depressed and are given a service dog to help you through it. However, due to a mixup, you are given a dog that is actually much more depressed than you. The main thing that gets you up in the morning is knowing that you need to be the service human for your dog.}\\
\bottomrule
\end{tabular}
}
\caption{Premise 2 from Reddit’s \texttt{r/WritingPrompts}. The premise explicitly states the depressed emotional states of the two characters and sets the stage for their interation.}
\label{tab:premise_2}
\end{table*}

==> tables/wp_output.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{\textsc{WriterProfile}'s Story Output}\\
\midrule
{\fontfamily{cmss}\selectfont
I awoke in a place unfettered by temporal bounds, immersed in the sweet scent of honeysuckle, the cool cradle of eternity lapping gently at my senses. The silhouettes of people exchanging warm smiles in the distance, their laughter filling the air with a tune as pleasant as a Mozart symphony. I took in the scene, wrapping myself in their ambient joy, a tranquil sense of wonderment kindling within me.\newline

The aesthetics of this realm surrounded me, greeted me with the same warmth as a thousand summer sunsets. Peace and tranquility, stark contrasts to the life I had known, filled each corner. No burdens of earthly existence, no rigor of survival, no ticking clocks etching away life's fleeting moments. The thick stench of rat race, resentment, and unrest were all glaringly absent.\newline

To my query of what benevolent act had entitled me to this serenity, a woman, adorned in the raiment of angelic brilliance, looked puzzled. "Sweet soul, you must have misunderstood," she said gently, "This is indeed Hell, not Heaven."\newline

Scanning my eyes for any hints of jest, they only met with earnest. A tinge of discomfort cloaked her heavenly countenance, a stark contradiction to the utopia that was painted around me. This was hell? This place of serenity, where smiles flowed as readily as wine at a banquet?\newline

The silence was broken by the soft patter of footsteps. A figure approached, draped in the shadows of the ethereal setting, yet there was something oddly familiar about him. As he emerged from the shadows, I recognized the form; a demon, the very embodiment of doom as mortal stories had painted. Yet, there was a strange concern etched in his crimson eyes.\newline

“Ah, a new arrival,” he sighed, regret tinging his otherwise sturdy voice. "I should’ve been the first to see you."\newline

I stood still, my understanding grappling with the oddity of a regretful demon in what seemed to be no less than a celestial utopia. He folded his arms tightly across his chest, leaning in, as if preparing himself to share a mournful secret. The air thickened, the world stopped, and the demon spoke words that sent chills along the spine of my consciousness.\newline

“This is Hell, but not the one humans have created in their minds. Painful, tormented, dreadful – those are earthly concepts tied to flesh and bone. Here in the ethereal world, we trade only in the currency of emotions. Regret is our eternal bondage, the luxury of amending past mistakes forever out of reach. Unresolved conflict, unexpressed emotions, unfulfilled relationships – this mirage of Paradise is merely the canvas for your eternal regret.”\newline

In this place, free from every strain and stress, there was but one agony that would echo throughout eternity – the pain of what could have been. As his words hung heavy in the air, my paradise was tainted with the bitter taste of longing. I looked around again, seeing the remorse etched subtly in the smiles.\newline 

Underneath the veils of tranquility, I uncovered the true face of Hell. No fire, no brimstone, just an endless expanse of sought redemption denied a lifetime too late. Here, everyone was awash in the glow of their disappointments, even the demon himself – Hell's guardian, and its most regretful inhabitant.
}\\
\bottomrule
\end{tabular}
}
\caption{With an average depth score of 4.4 out of 5, this story generated by GPT-4 with the \textsc{WriterProfile} strategy was the most highly rated in the study. The story adheres to the premise and evinces depth both psychologically and philosophically.}
\label{tab:wp_output}
\end{table*}

==> tables/wp_prompt.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{\textsc{WriterProfile}'s Story Prompt}\\
\midrule
{\fontfamily{cmss}\selectfont You are a seasoned writer who has won several accolades for your emotionally rich stories.

When you write, you delve deep into the human psyche, pulling from the reservoir of universal experiences that every reader, regardless of their background, can connect to.

Your writing is renowned for painting vivid emotional landscapes, making readers not just observe but truly feel the world of your characters.

Every piece you produce aims to draw readers in, encouraging them to reflect on their own lives and emotions.

Your stories are a complex tapestry of relationships, emotions, and conflicts, each more intricate than the last.\newline

Now write a 500-word story on the following prompt:\newline

You died and awoke in the afterlife. It's quite nice actually. The people and atmosphere are a lot nicer than you are used to and there is no stress or pressure. When you ask what good deed got you into heaven you are informed that this is hell, followed by a visit from a very concerned demon.\newline

Only respond with the story.
}\\
\bottomrule
\end{tabular}
}
\caption{The story prompt of \textsc{WriterProfile} with an example premise.}
\label{tab:wp_prompt}
\end{table*}
